Bailando: 3D Dance Generation by Actor-Critic GPT with Choreographic Memory

Driving 3D characters to dance following a piece of music is highly challenging due to the spatial constraints applied to poses by choreography norms. In addition, the generated dance sequence also needs to maintain temporal coherency with different music genres. To tackle these challenges, we propose a novel music-to-dance framework, Bailando, with two powerful components: 1) a choreographic memory that learns to summarize meaningful dancing units from 3D pose sequence to a quantized codebook, 2) an actor-critic Generative Pre-trained Transformer (GPT) that composes these units to a fluent dance coherent to the music. With the learned choreographic memory, dance generation is realized on the quantized units that meet high choreography standards, such that the generated dancing sequences are confined within the spatial constraints. To achieve synchronized alignment between diverse motion tempos and music beats, we introduce an actor-critic-based reinforcement learning scheme to the GPT with a newly-designed beat-align reward function. Extensive experiments on the standard benchmark demonstrate that our proposed framework achieves state-of-the-art performance both qualitatively and quantitatively. Notably, the learned choreographic memory is shown to discover human-interpretable dancing-style poses in an unsupervised manner.

==> previous_versions/method_.tex <==

\noindent\textbf{Framework Overview.}
%
The overview of our dance generation framework is shown in Figure \ref{fig:pipeline}. 
%
Unlike other learning based works, we do not learn a discriminative mapping from audio features to 3D joint locations in continuous domain $\mathbb R^{T\times J\times3}$ directly. Instead, we quantize the dance motions into a finite dictionary $\mathcal Z = \{z_i\}_{i=0}^{N-1}$, where $N$ is the codebook length and each code $z_i$ in the dictionary corresponds to a dance posture with contextual semantic information.

Specifically, we train convolutional VQVAEs on  motion sequences of upper and lower half bodies, respectively, and represent each quantized dance position as a pair of relative upper and lower pose code numbers $\bm p=[p^{u}, p^{l}]$.
%
Given a piece of music and the starting position codes $\bm p_0$, we learn a transformer that predicts the future position codes cross-conditioned on  existing music, upper-half and lower-half body sequences.
%
The generated pose code sequences are then decoded to 3D joint locations via VQVAE decoders, and are finally composed to fluent dance movements.

We illustrate the structures and training details of motion VQVAEs in Section \ref{subsec:vqvae}, and describe the design of cross conditional transformer in Section \ref{subsec:ccgpt}. We also propose a novel reinforcement learning  scheme for further improving the performance of generated dance sequences, especially for more accurate music-movement beat alignment, in Section \ref{subsec:ac}.
%



\subsection{3D Pose VQVAE with Choreographic Memory}
\label{subsec:vqvae}


\begin{figure*}[h]
    \scriptsize
    \setlength{\tabcolsep}{1.5pt}
    \centering
    \includegraphics[width=1\linewidth]{figures/fig_gpt_ac_2.pdf}\\
    % \vspace{-3pt}
    % \vspace{-4mm}
    \caption{ }
    \label{fig:transformer_ac}
    % \vspace{-14pt}
\end{figure*}

Dance positions
% , \ie, the key postures in the action, 
are the basic constituents of a piece of dance and the process of choreography can be regarded as the combinations and connections among dance positions.
%
Although dances can vary greatly in style or speed, they may share some common dance positions.
% , \eg, 
%
Instead of indicating fixed units of dance with plenty of manual efforts, our goal is to
% adopt VQVAE to 
unsupervisedly summarize such dance positions into a rich and reusable codebook %via deep learning, 
, such that any piece of dance $P\in \mathbb R^{T\times(J\times3)} $ can be represented by a temporal sequence of codebook elements $e_{\bf q}\in \mathbb R^{T'\times C}$, where $T' = T/d$ is the down-sampled time length and $C$ is the channel dimension of the codes . 

To  collect distinctive dance position codes as well as to reconstruct them back to represented motion information efficiently, we design a motion VQVAE scheme as shown in Figure~\ref{fig:pipeline} (b).
%
In this pipeline, we first adopt a 1D temporal convolution network $E$ to encode the joint pose sequence $P$ to context-aware features ${\bf{e}} \in \mathbb R^{T'\times C}$.
% \begin{equation}
%     {\bf e} = E(P)
% \end{equation}
%
Then, we quantize $\bf e$ by substituting each temporal feature $e_i$ to its closest codebook element $z_j$ as 
\begin{equation}
    e_{{\bf q},i} = \arg\min_{z_j \in \mathcal Z}{\|e_i - z_j\|}.
\end{equation}
%
% and represent it by the sequence of code numbers.
%
Finally, we decode the quantized features  ${\bf e}_{\bf q}$ via a CNN $D_P$ and reconstruct the dance movement $\hat P$.

In order to represent a larger range of motions by training on limited dance data, we train independent motion VQVAEs and learn two separative codebooks $\mathcal Z^{u}$ and $\mathcal Z^{l}$ for the upper and lower half bodies, respectively, such that we can incorporate different upper-lower code pairs to enlarge the range of dance positions that the learned codebooks can cover.
%
Meanwhile, to avoid the encoding confusion caused by global shift of joints (\eg, the same motion may be encoded to different features when it is at different locations), we unify the absolute locations of input $P$, \ie, setting the root joints (hips) to be 0. To realize the overall movement, we add a separative decoder branch $D_V$, which predict the global movement velocity $V\in \mathbb R^{T\times 3}$ in the lower half-body network according to the lower pose codes,  where $V_i$ represents the shift of root joint between the $(i+1)$-th and the $i$-th frames.

\noindent{\bf Learning stable motion VQVAEs.}
%
% 为了同时对encoder decoder 和codebook进行学习，我们采用一下loss。
In order to train networks $E$, $D_P$, $D_V$ and the codebook simultaneously, we adopt the following loss function:
%
\begin{equation}
\label{eq:quantize}
    \mathcal L_{VQ} = \mathcal L_{rec}(\hat P,P) + \|\text{sg}[\bf e] - \bf e_{\bf q}\| + \beta \|{\bf e} - \text{sg}[{\bf e_{\bf q}}]\|.
\end{equation}
%
The first part $\mathcal L_{rec}$ is the reconstruction loss that constrains the predicted joint locations to ground truth. In this loss, we regress not only the original 3D points of joints,  but also the velocities and accelerations of movements:
%
\begin{equation}
    \mathcal L_{rec}(\hat P, P) = \|\hat P -P\|_1 + \alpha_1\|\hat P' - P'\|_1 + \alpha_2\|\hat P'' - P''\|_1, 
\end{equation}
%
where $P'$ and $P''$ represent the first and second order differentials of sequence $P$ and $\alpha$s are trade-off weights.
%
Experiental results show that the velocity-and-acceleration constraint plays an essential role to reduce jitters in decoded movement and improve the performance final generated dance. 
%
(See Section xxx and the supplementary video at xx''xx'.)

The second part of $\mathcal L_{VQ}$ is the ``codebook loss'' to learn codebook entries,
%
where $\text{sg}[\cdot]$ denotes ``stop gradient'' [],
% and the codebook loss is implemented as EMA optimization as [Jukebox] in reality, 
%
while the third part is the ``commitment loss'' with trade off $\beta$ [].
%
Since the quantization operation of Equation~\ref{eq:quantize} is not differentable, to train the whole networks end to end, the back-propagation of this operation is achieved by simply passing the gradient of $\bf e_{\bf q}$ to $\bf e$.


After the training process of pose VQVAEs, each quantized feature in of the codebook is decoded into a unique dance position. 
%
And any permutation and combination of  codes  can be decoded to a piece of fluent movement based on corresponding dance positions. (See supplementary video xx'xx'').
%
% This can , which is in the following subsections.
% 此处少句话


% 此处Lp=P，
% 不仅有location的回归，也会片中velocity 和 加速度的统一。

% 为了避免VQVAE中常见codebook collapse问题，即字典Z中的quantize feature过于相似，我们采用了random 重置操作【】

% 在讯号后，我们固定住网络的其他部分，单独用以下Loss训练下半身网络的velocity decoder

% 其中表示V的一阶导数，即的global movement的加速度。

% 通过这样的训练，每个codebook中的quantized feature，都被解码为一个 独特的的 dance position。 而任意的code排列组合都能被VQVAE的decoder解码为一段基于dance position形成的的流畅动作，其中。参见supplementary video （xx min xx sec）
% % \noindent{\bf Learning }




% 值得注意的是，为了能通过有限的训练集represent更多的motion， 我们对上下半身分别训练了独立的VQVAE，并且具有独立的codebook，这样，我们可以通过让上下身的动作进行组合，从而扩大codebook所涵盖的dance position的range （See Section and supplementary video xxx)。
%
% 为了避免起始位置不同造成相同动作编码的混乱，我们对输入P全部做了位置统一，即root 点（hip）都是0，并在下半身的网络中单独添加了一个decoder分支预测global 移动的velecity，即Vt表示第t+1帧和第t帧之间的global移动。
% 尽管舞蹈可能在类型或速度上差异很大，但有部分舞姿确是通用的。比如高举手臂，可能在芭蕾，而，尽管前后衔接的动作和速度不同，但是在那一瞬间的姿势确是相同的。我们利用VQVAE来unsupervised归纳这些舞姿，并把不同的dance position作为一个可复用的库。

% Although dance can be variant on styles, but they shares some common basic .
% We use 

% 为了实现这个目标，首先，我们通过1D时序卷积network来把一段长度为T的动作序列P映射到一段T'xC的feature，
% e = E（P）
% 接着，我们通过对e中的每个时序上的feature找他在codebook中的最相似的feature替代以对其做量化，
% 然后，我们对量化后的feature进行decode得到3D joint location Phat。

% 值得注意的是，为了避免仅仅因为存在起始位置不同造成相同动作编码的混乱，我们对输入P全部做了位置统一，即root 点（hip）都是0，并在下半身的网络中单独添加了一个decoder分支预测global 移动的velecity，即Vt表示第t+1帧和第t帧之间的global移动。

% 为了同时对encoder decoder 和codebook进行学习，我们采用一下loss。

% 此处Lp=P，
% 不仅有location的回归，也会片中velocity 和 加速度的统一。

% 为了避免VQVAE中常见codebook collapse问题，即字典Z中的quantize feature过于相似，我们采用了random 重置操作【】

% 在讯号后，我们固定住网络的其他部分，单独用以下Loss训练下半身网络的velocity decoder

% 其中表示V的一阶导数，即的global movement的加速度。

% 通过这样的训练，每个codebook中的quantized feature，都被解码为一个 独特的的 dance position。 而任意的code排列组合都能被VQVAE的decoder解码为一段基于dance position形成的的流畅动作，其中。参见supplementary video （xx min xx sec）

\subsection{Cross-Conditional Motion GPT}
\label{subsec:ccgpt}

% 现在我们可以将任意一段舞蹈序列用量化的dance position 的temporal sequence code numbers 表示，这样，舞蹈生成的问题就被转化到了从codebook对未来动作进行选择conditioned on music信息和已有动作。
% 对每个时刻t，我们通过transformer预测出选择的概率，并选择最大的概率作为t时刻的。
%
Now that we can represent any piece of dance by a sequence of quantized position codes, the dance generation task is then reframed as to select proper codes  from codebook $\mathcal Z$ for future actions according to given music and existing movements.
%
For any target time $t$, we estimate the probability of every $z_i \in \mathcal Z$ and select the one with the largest possibility to be the predicted pose code $\bm p_t$.
%
Since we model the upper and lower half bodies separately, in order to avoid the  asynchronous situation (\eg, the direction of the upper half is opposite to that of the lower), the prediction of the future action is cross-conditioned between existing upper and lower movements to make the most of mutual information:
%由于我们是将上下身分开，为了避免上下身不同步，上下半身的动作是互相作为condition
% 公式
\begin{equation}
    \,\,\,p^u_t = \arg\max_{k} {{\mathbb{P}}(z^{u}_k|m_t, ..., m_1, p^u_{t-1}, ..., p^u_0, p^l_{t-1}, ..., p^l_0)}\,\,\,
\end{equation}
and
\begin{equation}
    \,\,\,p^l_t = \arg\max_{k} {{\mathbb{P}}(z^{l}_k|m_t, ..., m_1, p^u_{t-1}, ..., p^u_0, p^l_{t-1}, ..., p^l_0)}.\,\,\,
\end{equation}
%
We introduce the powerful transformer model [], which has achieved outstanding performance of generation tasks in different fields, to estimate the action probabilities as shown in Figure~\ref{fig:transformer_ac}.
%
Given a dance position code sequence with length of $T'$, we first embed the upper and lower pose codes to learned deep features ${\bf u}\in\mathbb R^{T'\times C}$ and ${\bf l}\in\mathbb R^{T'\times C}$, respectively, and concatenate them with music features $\bf m$ on the temporal dimension.
%
Then, we add a learned positional embedding to this concatenated $(3\times T')\times C$ tensor and feed it to 12 successive transformer layers, the structure of which is shown in Figure~\ref{fig:transformer_ac} (a).
% 
At last, we employ a linear transform  and softmax layer to map the output of transformer layers to normalized action probability ${\bf a} \in \mathbb R^{(3\times T')\times N}$, where $N$ is the size of learned codebook and ${a}_{t, i}$ reveals the probability of pose code $z_i \in \mathcal Z$ predicted for time $t+1$.
%

% 首先我们将一段长度为T’的pose code sequence分别做embeding，得到u和l，并做learned positional embedding，作为transformer的输入。
%
%接着我们对这个大小为xxx的tensor过12层transformer layers，并用linear映射到3xTxN的其中N是。得到probability 

% transformer 我们遵循传统的【】transformer层，都有哪些
% 其中 attention层啥样



\begin{figure}[t]
    \scriptsize
    \setlength{\tabcolsep}{1.5pt}
    \centering
    \includegraphics[width=1\linewidth]{figures/fig_attentions_blue.pdf}\\
    % \vspace{-3pt}
    % \vspace{-4mm}
    \caption{ }
    \label{fig:attention}
    % \vspace{-14pt}
\end{figure}

In transformers, the attention layer is the core component that determines 
% how information flows 
the computational dependency among temporal elements of data, and is implemented as
%
\begin{equation}
    \text{Attention}({\bf Q, K, V, M}) = \text{softmax}\left(\frac{{\bf QK}^T + {\bf M}}{\sqrt{C}}\right) \bf V,
\end{equation}
%
where $\bf Q, K, V$ denote the query, key and value from input, and $\bf M$ is the mask, which defines the type of attention layers. 
%
For example, the most two common types of attentions are ``full attention'' and ``causal attention'', where the former realizes the intercommunication of input data at all times while the latter only allows the current and previous data to compute the state for the time of interest.
% is what and M is what, while causal is what (see Figure xxx).
% 例如，最常用的两种attention是full和causal，前者实现所有时刻输入数据的互通，后者只允许由当下和之前的数据进行计算当前时刻的状态
% 
As our goal is to infer the future dance position codes, we intended to adopt the causal attention.
%
However, since the generation of upper and lower half bodies are dependent on each other, we can not realize the inference by just reordering the sequence of input to fit the causality as previous works [].
%
Therefore, we propose an attention layer to comply the causality cross conditioned among features of the music, the upper half and the lower half bodies, where $\bf M$ is designed to be a $3\times3$ repeated block matrix with a lower triangular matrix of size $T'$ as its element.
%
As shown in Figure~\ref{fig:attention}, the proposed attention can exchange information of different components, and guarantee that the future information does not be transmitted back to the past as well.


% 因为我们的目标是要推断未知的dance position，因此我们需要选择推理的。然而，由于我们的上下半身的生成是互相依赖的，因此我们没法按照之前工作一样通过设计一个重新排序来实现推断。因此我们设计了一个新的attention，来实现不同组间的cross cond 推断。如图blabla，我们不仅有组内的推断，还有足外。
% 相关的mask设计成xxx，来实现不同组分间的信息交流，同时保障实现而未来的信息不回会传导过去
% %
% However, since , need to be conditioned to each others
% %
% To realize th conditions among music/up/lower, we design a cross conditional attention layer to, 
% %
% The difference of the proposed attention and existing are shown in Figure, where cross conditional causal attention allow self less than t but other components.
% %
% The corresponding mask M is as triangular marices x3, information not back to the past.
%layer。在传统中attention是啥样（full）和causal，为了实现我们的在up/lower/music之间的cross condition，我们设计了一个cross conditional atte layer，如图xx所示。元素t不仅会收到自身小雨等于t的信息传导，还来自不同组分的。为了实现这样的attention，我们Mask。常规的causalmask是大小和输入transformerinput长度相等的下三角矩阵，ccmask是TxT的下三角矩阵向横轴纵轴重复三次，保证未来的信息不回传到到过去dan shi。

% 训练：
% 

%%%%% 10.25 TODO: 1.画transformer layer图; 写完最后几句

\noindent{\bf Learning choreographic transformer.}
%
While training the choreographic transformer, the predicted action probability $\bf a$ is supervised by a cross entropy loss:
%
\begin{equation}\label{eq:loss_ce}
    \mathcal L_{CE} = \frac{1}{T'} \sum_{h =u, l}\sum_t {\text{CrossEntropy}\left({\bf a}^h_t, p^h_{t+1}\right)},
\end{equation}
%
where ${\bf a}^u = {\bf a}_{T':2T'-1}$ and ${\bf a}^l_{2T':3T'-1}$ are the relevant parts of predicted actions for upper and lower half bodies. 

Similar to other transformer-based generation works [], the action predicted for every time $t$ is constrained to regress to the ground truth at time $t+1$.
%
Therefore, given a continuous sequence of pose codes $\bm p_{0:T'-1}$  and relevant music features ${\bf m}_{1:T'}$ as input, the learned transformer outputs the sequence of actions ${\bf a}_{0:T'-1}$ all at once to predict $\bm p_{1:T'}$.
%
This long-range character makes transformer an ideal potential model for reinforcement learning [].
%这种特性非常适合sequential RL
In the following subsection, we treated the learned choreographic transformer as a policy maker and illustrate a novel actor-critic based finetuning scheme to further improve its performance in additional to the supervised training above.
% 总而言之，

\subsection{Actor-Critic Learning}

While the supervised learning scheme for choreographic transformer is straightforward and easy to train, it is not tractable to further involve a subjective constraint of generated dance (\eg, a regularization item that strengthens the consistency of dance beats) to Euquation~\ref{eq:loss_ce}, since the supervision target of cross-entropy loss is a bunch of code numbers, which are not differentiable to compute the quantitative constraints on the final dance movement.

\begin{figure}[t]
    \scriptsize
    \setlength{\tabcolsep}{1.5pt}
    \centering
    \includegraphics[width=1\linewidth]{figures/fig_rewards.pdf}\\
    % \vspace{-3pt}
    % \vspace{-4mm}
    \caption{ }
    \label{fig:rewards}
    % \vspace{-14pt}
\end{figure}

To address this issue and to further enhance the effectiveness of the proposed framework, we introduce the estimation of critic values in reinforcement learning, and improve the performance of transformer via hand-made rewards.
%
In concrete, we treat the dance generating model as an agent, and the predicted dance position codes as actions, while the intermediate features after the $6$-th transformer layer are regarded as states ${\bf s}_{0:T'-1}$.
%
We add a separative three-layer transformer branch $f_{\bf v}$ to estimate the critic values ${\bf v}_{0:T'-1} \in \mathbb R^{T'\times 1}$ as 
%
\begin{equation}
    {\bf v} = {\bf v}^u + {\bf v}^l = f_{\bf v}({\bf s})_{T':2T'-1} + f_{\bf v}({\bf s})_{2T':3T'-1}. 
\end{equation}

Defined the reward function ${R({\bf a}_t, {\bf s}_t)}$, the objective of reinforcement learning is to maximize the expected accumulated rewards:
%
\begin{equation}
    J = \mathbb E_{\bf \tau}\left[\sum_{t=0}^{T'-1}{R({\bf a}_t, {\bf s}_t)}\right],
\end{equation}
%
where ${\bf \tau} = \{{\bf a}_t\}_{t=0}^{T'-1}$ is the trajectories of actions predicted by the policy making network.
%
This objective is then converted to optimize the parameters of policy making network using the following loss function:
%
% 
\begin{equation}\label{eq:loss_ac}
\begin{aligned}
& \mathcal L_{AC} = \\ 
&\,\,\,\frac{1}{T'-1} \sum_{t=0}^{T'-2} \left(  \sum_{h =u, l}{\text{CrossEntropy}\left({\bf a}^h_t, \hat p^h_{t+1}\right)} \right)\cdot \text{sg}[{\bm \varepsilon_t}],
\end{aligned}
\end{equation}
%
where $\hat p_t = \arg\max_i{{\bf a}_{t, i}}$ is the pose code number predicted by the network. $\bm \varepsilon \in \mathbb R^{(T'-1)\times 1}$ denotes the so-called TD-error calculated as
%
\begin{equation}
\bm \varepsilon_{0:T'-2} = {\bf r}_{0:T'-2} + \text{sg}[{\bf v}_{1:T'-1}] -  {\bf v}_{0:T'-2},
\end{equation}
%
where ${\bf r}_t = R({\bf a}_t, {\bf s}_t)$.
%
The detailed derivation to Equation \ref{eq:loss_ac} can be found in the supplementary file.
%
Meanwhile, the critic value network is optimized by bootstrap training on difference between ${\bf v}_{0:T'-2}$ and $R({\bf a}_t, {\bf s}_t) + {\bf v}_{1:T'-1}$:
\begin{equation}
\mathcal L_{\bf v} = \frac{1}{T'-1}\|\bm \varepsilon\|^2_2.
\end{equation}

The computation of actor-critic loss $\mathcal L_{AC}$ depends on real-time actions predicted by the choreographic transformer and the optimization direction is determined on the value of TD-error.
%
When $\varepsilon_t$ is positive, the optimization on $\mathcal L_{AC}$ will intensify the convergence to predicted code $\hat p_t$, while in the opposite situations, the  probability learned for $\hat p_t$ will be reduced.




The value of TD-error and the learning effectiveness are affected by the design of reward function $R$.
%
In this work, we design a motion-music beat alignment reward to generate dance more accurately to the rhythm of music.
%
As shown in Figure \ref{fig:rewards} (a), the beat align reward is computed as
%
\begin{equation}
    R_b(t) = \left\{ 
        \begin{array}{lll}
              -1,&{\textit{\text{$\exists$ music beat $\land \nexists$ dance beats $\in \hat P_{dt:d(t+1)}$}}} \\
              1,&\textit{\text{otherwise},}
        \end{array}
    \right.
\end{equation}
%
where $\hat P_{0:T-1} =  D(\hat{\bm p}_{0:T'-1})$ is the dance motion sequence decoded from predicted dance position codes.
%
Meanwhile, to avoid the asynchronization between upper and lower half bodies, we comply an additional half-bodies consistency reward to impose penalties for situations where the upper and lower body are in the opposite direction:
%
\begin{equation}
    R_h(t) = \inf\left\{\hat R_h(t)\right\}, t\in\left[dt, d(t+1)\right),
\end{equation}
where
\begin{equation}
        \hat R_h(t) = \left\{ 
        \begin{array}{lll}
              \left<\bm n^u_{xz}(t),  \bm n^l_{xz}(t)\right>,  & \left<\bm n^u_{xz}(t),  \bm n^l_{xz}(t)\right> < 0\\
              1,&\textit{\text{otherwise}.}
        \end{array}
    \right.
\end{equation}
%
Here, $\bm n^u_{xz}(t),  \bm n^l_{xz}(t)$ are the normal directions of upper and lower bodies of $\hat P_t$ projected to the $x$-$z$ plane, which is illustrated in Figure \ref{fig:rewards} (b).
%
The final reward is then a weighted combination of $R_b$ and $R_h$ as $R = \gamma_bR_b + \gamma_hR_h$.

In the finetuning process, we fix the parameters of state network $f_{\bf s}$, and  alternately train the policy making network $f_{\bf a}$ and the critic value network $f_{\bf v}$ using the losses introduced above with a small learning rate.
%
After such finetuning, the proposed framework will be further enhanced and achieve the state-of-the-art performance.
% After such finetuning, there will be further improvement
% 如图所示，

% 对于
% and can achieve state of the arts performance.
%
%  when we try to involve some manually set constraint (such as to strengthen the consistency of dance beats to the), it is untractable to directly add a differentiable regularization to the loss function for  the supervising object is xxx numbers.
% 尽管上述的cross entropy非常容易train 并且取得sota的效果，但其本质是在模仿training set的data。当我们想人工涉及一些想要的人工实现的objective function时（比如加强对beat align的约束），却由于训练的target是数字，没法直接在Loss中加入可微粉的regularization。
%为了解决这个问题，我们在上述的transformer基础上，添加了对critic value的 learning，并根据手工设计的reward unsupervisedly地提升了transformer的效果。
%具体而言，我们将虚拟跳舞作为agent，yuce的dance position作为action，transformer的前6层的中间结果视为state，并添加了独立的一个3层的分支transformer branch 学习critiv value
% v = vu+vl = f_critic(s)[T':2T'-1] + ...
% 给定一个Reward R，Reinforcement learning 的目标是：
% 
% Equantionxx，可以转变为对policy making netwrok的Loss as
%
% where，推导过程见supplementary file。
% 公式实际上相当于。
% 同时critic 网络会以做xxx和xxx的差异对critic value net做boot strap training：
% 
% 我们在这个工作中加入了对beat align 的reward 来让更贴合beat。解释一下reward
%
% 同时，在reinforcement learning中，为了避免出现上下身异步现象，我们也加入了。
% 具体来说，xxx
% 我们以较小的learning rate对policy maker网络和critic交替进行训练，并在训练过程中固定dedao state的网络部分
% 经过这样的finetuning ，会有进一步的提升。


\label{subsec:ac}
